Drive the Thoughts: Runtime Monitoring of VLA Reasoning-Trajectory Consistency

While machine learning models help autonomous vehicles (AVs) navigate complex environments, their black-box nature complicates validation and verification (V&V). Vision-language-action (VLA) models offer a unique opportunity: alongside trajectories, they generate an explicit chain-of-thought (CoT) explaining their decisions. We posit that this CoT can serve as a candidate specification to cross-check trajectories and expose unsafe behavior. To assess this, we curate DriveAlignBench, a dataset of 150 CoT-trajectory pairs from NVIDIA's Alpamayo 1.5 VLA, manually annotated for CoT reliability, CoT-trajectory consistency, and trajectory safety. We find that 33.3% of CoTs are unreliable, and among reliable CoTs, 26% have inconsistent trajectories. To detect these cases, we propose integrating a CoT-trajectory consistency check into a runtime monitor. This check is nontrivial because CoTs express open-vocabulary, scene-relative maneuvers, while trajectories are low-level ego-motion sequences whose semantics depend on road geometry and motion context. To bridge this gap, we develop a family of automated consistency monitors. The strongest, the lane-aware monitor, adds lane-relative evidence to the input of the judge model scoring consistency. This raises F1 across all four evaluated judges from 0.56-0.62 with raw waypoints to 0.65-0.82, showing that evidence representation improves detection across judges. Moreover, for reliable CoTs, inconsistency is associated with unsafe behavior: 27% of human-labeled inconsistent trajectories are unsafe compared to 3% of consistent ones, and the lane-aware monitor flags most of these unsafe cases. We release DriveAlignBench, the monitor implementations, and per-run results at https://github.com/less-lab-uva/drive-the-thoughts.

==> sections/fig_consistency_examples.tex <==
\begin{figure}[t]
\centering
\definecolor{conbad}{HTML}{B2182B}
\setlength{\fboxrule}{1pt}\setlength{\fboxsep}{0pt}
\fcolorbox{conbad}{white}{\includegraphics[height=2.35cm]{figures/cot_cons_b_cam.jpg}}\hspace{1.5pt}%
\fcolorbox{conbad}{white}{\includegraphics[height=2.35cm]{figures/cot_cons_b_traj.png}}
\caption{An \textsc{inconsistent} and \textsc{unsafe} pair from the reliable
subset: front camera (left) and planned trajectory $\tau$ in bird's-eye view
(right; ego in green, path in orange, lanes in blue). The CoT says ``Change lane
to the left due to slower vehicles ahead...'', but $\tau$ swings left across the
intersection into oncoming traffic. The two labels are annotated independently and
need not coincide.}
\label{fig:consistency-examples}
\end{figure}

